Reasoning-as-Logic-Units: Scaling Test-Time Reasoning in Large Language Models Through Logic Unit Alignment

Chain-of-Thought (CoT) prompting has shown promise in enhancing the reasoning capabilities of large language models (LLMs) by generating natural language (NL) rationales that lead to the final answer. However, it struggles with numerical computation, which has somehow led to the development of program-aided techniques. Despite their potential, a persistent challenge remains: inconsistencies between LLM-reported reasoning steps and the logic in generated programs, which we term ``reasoning hallucinations." This stems from the inherent ambiguities of NL and the statistical nature of LLMs, which often lack rigorous logical coherence. To address this challenge, we propose a novel test-time scaling framework, Reasoning-as-Logic-Units (RaLU), which constructs a more reliable reasoning path by aligning logical units between the generated program and their corresponding NL descriptions. By decomposing the initially generated program into discrete units using static analysis, RaLU engages in an iterative dialogue with the LLM to judge, refine, and explain each unit. A rewind-and-correct mechanism ensures alignment between code statements and task requirements in each unit, ultimately forming a cohesive reasoning path under the program's logic, from which the model reaches a final solution. Our experiments demonstrate that RaLU significantly outperforms existing baselines in mathematical reasoning (GSM8K, MATH) and algorithmic reasoning (HumanEval+, MBPP+), underscoring its potential to advance LLM reasoning and programming by offering enhanced accuracy and interpretability.

==> tables/3_token.tex <==
\begin{table*}[htb]\centering
    \caption{Average token consumption per task of \tool and baselines among the four benchmarks. In each cell, $i/o$ denotes the average input and output token consumption, respectively. \tool consumes 15x tokens compared to CoT, while save xx tokens compared to multi-path reasoning baselines such as Self-Check and ToT.}
    \begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{*{11}{c}}
    \toprule
    Task & Direct & CoT & ToT & PoT & SR & SC & SCal & SCheck & SD & \tool \\
    \cmidrule{1-11}
    Math & 111/15 & 222/177 & 15704/2269 & 334/238 & - & 4172/405 & 668/239 & 9551/6580 & -& 3647/375 \\
    Code & 165/67 & 215/216 & 25303/3327 & - & 1624/460 & 4740/883 & 631/240 & - & 273/364 & 3465/592\\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
      %   \begin{tablenotes}
      %   \footnotesize
      %   \item[$\star$] Only the result on \dfj 1.2 is available. 
      %   \item[$\dagger$] The result is obtained from 665 sampled bugs.
      %   \item[$\ddagger$] We randomly select 100 plausible patches to check their correctness because of the huge number of plausible patches.
      % \end{tablenotes}
    
\vspace{-0.1in}
\label{tab:exp:token}
\end{table*}

